STELLA: Continual Audio-Video Pre-training with Spatio-Temporal Localized Alignment

Continuously learning a variety of audio-video semantics over time is crucial for audio-related reasoning tasks in our ever-evolving world. However, this is a nontrivial problem and poses two critical challenges: sparse spatio-temporal correlation between audio-video pairs and multimodal correlation overwriting that forgets audio-video relations. To tackle this problem, we propose a new continual audio-video pre-training method with two novel ideas: (1) Localized Patch Importance Scoring: we introduce a multimodal encoder to determine the importance score for each patch, emphasizing semantically intertwined audio-video patches. (2) Replay-guided Correlation Assessment: to reduce the corruption of previously learned audiovisual knowledge due to drift, we propose to assess the correlation of the current patches on the past steps to identify the patches exhibiting high correlations with the past steps. Based on the results from the two ideas, we perform probabilistic patch selection for effective continual audio-video pre-training. Experimental validation on multiple benchmarks shows that our method achieves a 3.69%p of relative performance gain in zero-shot retrieval tasks compared to strong continual learning baselines, while reducing memory consumption by ~45%.

==> defs.tex <==

%\usepackage[numbers, sort&compress]{natbib}

\usepackage{pifont}
\usepackage{amsmath, amssymb, bm, amsthm}
\usepackage{mathrsfs} 
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{color}
\usepackage{booktabs}
\usepackage{array}
\usepackage{tabularx, booktabs, multirow}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}


\usepackage[capitalize,nameinlink]{cleveref}


%\numberwithin{equation}{section}
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{defn}{Definition}[section]
\newtheorem{lem}{Lemma}[section]
%\newtheorem{cor}{Corollary}[section]
\newtheorem{cor}{Corollary}
%\newtheorem{prop}{Proposition}[section]
%\theoremstyle{definition}
%\newtheorem{algorithm}{Algorithm}[section]
%\newtheorem{example}{Example}[section]


\newcommand{\dee}{\mathrm{d}}
\newcommand{\grad}{\nabla}

\DeclareMathOperator{\ber}{Ber}
\DeclareMathOperator{\gammadist}{Gamma}
\DeclareMathOperator{\betadist}{Beta}
\DeclareMathOperator{\dir}{Dir}
%\DeclareMathOperator{\cat}{cat}
\DeclareMathOperator{\expon}{expon}
%\DeclareMathOperator{\unif}{unif}
%\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\sgm}{sgm}
\DeclareMathOperator{\frob}{{F}}
\DeclareMathOperator{\softmax}{{softmax}}
\DeclareMathOperator{\var}{{Var}}
\DeclareMathOperator{\diag}{{diag}}
\DeclareMathOperator{\softplus}{{Softplus}}
\DeclareMathOperator{\pool}{{StatisticsPooling}}

\newcommand{\normal}{\mathcal{N}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\card}[1]{\vert {#1} \vert}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}
\newcommand{\Indicator}[1]{\mathds{1}_{\{#1\}}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
\newcommand{\iid}{i.i.d.}

\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
%%\newcommand{\E}{{\mathbb{E}}}
\newcommand{\Real}{{\mathbb{R}}}
\newcommand{\calP}{{\mathcal{P}}}
\newtheorem{observation}{Observation}

\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bof}{\mathbf{f}}
\newcommand{\bhy}{\widehat{\by}}
%\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bhW}{{\widehat{\bW}}}
\newcommand{\btW}{{\widetilde{\bW}}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}
\newcommand{\noise}{{\boldsymbol{\varepsilon}}}

\newcommand{\ts}{{\tau}}

\newcommand{\bee}{\begin{eqnarray}}
\newcommand{\eee}{\end{eqnarray}}



==> materials/figures/supplement_figure_dataset_stat.tex <==
\begin{figure*}[t]
    \centering
    
    \begin{minipage}{0.48\textwidth}
    \centering
    \setlength{\tabcolsep}{-1pt}{%
    \includegraphics[width=1.0\linewidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/dataset_stat/vggsound_stat.pdf}
    }
    \textbf{(a) Continual-VS statistics}
    \end{minipage}
    \hspace{0.5cm}
    \begin{minipage}{0.46\textwidth}
    \centering
    \setlength{\tabcolsep}{-1pt}{%
    \includegraphics[width=1.0\linewidth, trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/dataset_stat/audioset_stat.pdf}
    }
    \textbf{(b) Continual-AS statistics}
    \end{minipage}
    % \vspace{0.15in}

    \caption{\small \textbf{Stastics of Audio-Video datasets} \textbf{(a)}: We split the VGGSound into 8 tasks, where each subset dataset consists of similar amounts of video clips. 
    \textbf{(b)}: We split the AudioSet into 7 tasks. Unlike the VGGSound dataset, the number of video clips varies significantly for each task.
    }
    \label{fig:dataset_stat}
\end{figure*}

==> materials/figures/supplement_figure_no_mae.tex <==
\begin{figure*}
    
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth]{figures/classification/no_mae/no_mae_cls_avg_acc.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/classification/no_mae/no_mae_cls_avg_forgetting.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/classification/no_mae/no_mae_Sports_Classification_Acc.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/classification/no_mae/no_mae_Music_Classification_Acc.pdf}\\
        \multicolumn{2}{c}{\textbf{(a) Comparison of classification results}} &
        \multicolumn{2}{c}{\textbf{(b) Task-wise task-specific classification result}}\\
    \end{tabular}}
\vspace{-0.05in}
 \caption{\textbf{Audiovisual classification results without MAE loss term.} \textbf{(a)}: We compare the audiovisual classification results from the models with the MAE loss term (\textit{Finetune}, \textit{ER}) and the models without it (\textit{Finetune-no-mae}, \textit{ER-no-mae}). \textbf{(b)}: We visualize changes in the task-specific average classification accuracy of the sequentially pre-trained model without the MAE loss term.
 }
    \label{fig:no_mae_result}
\vspace{-0.05in}
\end{figure*}

==> materials/figures/supplement_figure_scl_ucl.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}{c}
    \includegraphics[width=1.0\linewidth]{figures/concept_figure/scl_ucl.pdf}
    \end{tabular}
    \vspace{-0.15in}
    \caption{\small \textbf{Comparison with supervised continual learning and continual pre-training}: We illustrate the difference between the supervised continual learning setup and the continual pre-training setup that we used in our experiments.}
    \label{fig:scl_ucl}
\end{figure*}

==> materials/tables/supplement_table_classification_table.tex <==
\begin{table}[t]
    \centering
    \vspace{-0.05in}
    \caption{\small \textit{Continual-VS} \& \textit{Continual-AS} audiovisual classification task. The best and the second best results are highlighted in \textbf{bold} and \underline{underline}, respectively.}
    \vspace{-0.1in}
    \begin{adjustbox}{width=\linewidth}
    \renewcommand{\tabcolsep}{2.4pt}
    \begin{tabular}{ll cc cc}
        \toprule
        & {\textbf{Method}}&\multicolumn{2}{c}{\textbf{Continual-VS (Acc)}}&\multicolumn{2}{c}{\textbf{Continual-AS (mAP)}} \\
        & & $\mathcal{A} \uparrow$ & $\mathcal{F} \downarrow$ & $\mathcal{A} \uparrow$ & $\mathcal{F} \downarrow$ \\
        \midrule
        \parbox[t]{2mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{Classification}}}
        & \footnotesize Finetune &
        {\footnotesize 57.01~\tiny{($\pm$ 0.31)}} & {\footnotesize 2.15~\tiny{($\pm$ 0.51)}} &
        {\footnotesize 63.98~\tiny{($\pm$ 0.18)}} & {\footnotesize 2.12~\tiny{($\pm$ 0.15)}} \\
        & \footnotesize ER &
        {\footnotesize 58.30~\tiny{($\pm$ 0.13)}} & {\footnotesize 1.28~\tiny{($\pm$ 0.07)}} &
        {\footnotesize 65.10~\tiny{($\pm$ 0.32)}} & {\footnotesize 1.11~\tiny{($\pm$ 0.25)}} \\
        & \footnotesize MIR &
        {\footnotesize 58.07~\tiny{($\pm$ 0.30)}} & {\footnotesize 1.49~\tiny{($\pm$ 0.19)}} &
        {\footnotesize 65.17~\tiny{($\pm$ 0.20)}} & {\footnotesize 0.86~\tiny{($\pm$ 0.06)}} \\
        & \footnotesize DER++ &
        {\footnotesize 58.30~\tiny{($\pm$ 0.19)}} & {\footnotesize 1.27~\tiny{($\pm$ 0.51)}} &
        {\footnotesize 65.17~\tiny{($\pm$ 0.44)}} & {\footnotesize 1.39~\tiny{($\pm$ 0.45)}} \\
        & \footnotesize GMED &
        {\footnotesize 58.21~\tiny{($\pm$ 0.18)}} & {\footnotesize 1.16~\tiny{($\pm$ 0.38)}} &
        {\footnotesize 65.24~\tiny{($\pm$ 0.07)}} & {\footnotesize \underline{0.82}~\tiny{($\pm$ 0.17)}} \\
        & \footnotesize CLS-ER &
        {\footnotesize 58.34~\tiny{($\pm$ 0.14)}} & {\footnotesize 1.22~\tiny{($\pm$ 0.04)}} &
        {\footnotesize 65.21~\tiny{($\pm$ 0.08)}} & {\footnotesize 1.17~\tiny{($\pm$ 0.28)}} \\
        & \footnotesize LUMP &
        {\footnotesize 58.03~\tiny{($\pm$ 0.24)}} & {\footnotesize 1.17~\tiny{($\pm$ 0.14)}} &
        {\footnotesize 65.38~\tiny{($\pm$ 0.23)}} & {\footnotesize 1.24~\tiny{($\pm$ 0.23)}} \\
        & \footnotesize ESMER &
        {\footnotesize 58.49~\tiny{($\pm$ 0.13)}} & {\footnotesize 0.95~\tiny{($\pm$ 0.07)}} &
        {\footnotesize \underline{65.76}~\tiny{($\pm$ 0.18)}} & {\footnotesize 1.13~\tiny{($\pm$ 0.21)}} \\
        \cmidrule{2-6}
        & \footnotesize \cellcolor{gg}STELLA (Ours)&
        {\footnotesize \cellcolor{gg}\underline{58.65}~\tiny{($\pm$ 0.28)}} & {\footnotesize \cellcolor{gg}\textbf{0.64}~\tiny{($\pm$ 0.27)}} &
        {\footnotesize \cellcolor{gg}65.66~\tiny{($\pm$ {0.16})}} & {\footnotesize \cellcolor{gg} 0.89~\tiny{($\pm$ 0.23)}} \\
        & \footnotesize \cellcolor{gg}STELLA+ (Ours)&
        {\footnotesize \cellcolor{gg} \textbf{59.07}~\tiny{($\pm$ 0.14)}} & {\footnotesize \cellcolor{gg} \underline{0.80}~\tiny{($\pm$ 0.34)}} &
        {\footnotesize \cellcolor{gg} \textbf{66.05}~\tiny{($\pm$ 0.28)}} & {\footnotesize \cellcolor{gg} \textbf{0.78}~\tiny{($\pm$ 0.27)}} \\
        \cmidrule{2-6}
        & \footnotesize Multitask &
        {\footnotesize 59.90~\tiny{($\pm$ 0.35)}} & $-$ &
        {\footnotesize 67.81~\tiny{($\pm$ 0.12)}} & $-$ \\
        % \cmidrule{2-6}
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:classification_table}
    \vspace{-0.15in}
\end{table}

==> materials/tables/supplement_table_dataset_config.tex <==
\resizebox{1.0\textwidth}{!}{%
\addtolength{\tabcolsep}{-2.8pt}
\renewcommand{\arraystretch}{1.2}
\renewcommand{\tabcolsep}{3pt}
\begin{tabular}{l cccccccc ccccccc}
    \toprule
     & \multicolumn{8}{c}{VGGSound} & \multicolumn{7}{c}{AudioSet} \\
    \midrule
    {Category} & {Sports} & {Music} & {Vehicle} & {People} & {Animals} & {Home\&nature} & {Others part1} & {Others part2} & {Music} & {Human} & {Vehicle} & {Home} & {Nature} & {Others} \\
    \cmidrule{2-16}
    Train & 7737 & 8000 & 8000 & 8000 & 8000 & 6807 & 6639 & 5390 & 29144 & 30073 & 25865 & 13924 & 15373 & 15848 & 25416 \\
    Evaluate & 886 & 907 & 906 & 862 & 873 & 837 & 863 & 810 & 1188 & 1523 & 1011 & 680 & 864 & 403 & 1585 \\
    Retrieval & 119 & 288 & 139 & 209 & 317 & 92 & 85 & 104 & 130 & 145 & 126 & 103 & 81 & 42 & 175 \\
    \bottomrule
\end{tabular}}

==> materials/tables/supplement_table_forget_robust_method.tex <==
\begin{wraptable}{t}{0.35\textwidth}
    \centering
    \caption{\small Retrieval result by prune methods pre-trained on VGGSound dataset.}
    \vspace{-0.1in}
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{l cc cc}
        \toprule
        Method & \multicolumn{2}{c}{A$\rightarrow$V} & \multicolumn{2}{c}{V$\rightarrow$A} \\
        & $\mathcal{A} \uparrow$ & $\mathcal{F} \downarrow$ & $\mathcal{A} \uparrow$ & $\mathcal{F} \downarrow$ \\
        \midrule
        Random & 3.30 & 9.26 & 3.13 & 8.83 \\
        Attention & 12.18 & 6.27 & 12.08 & 6.82 \\
        \textbf{OURS} & \textbf{13.88} & \textbf{4.85} & \textbf{14.02} & \textbf{4.99}  \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:forget_robust_prune_method}
\end{wraptable}
